Simon's model does not produce Zipf's law: The fundamental rich-get-richer mechanism for any power-law size ranking

Many complex systems are composed of disparate, interacting types of varying sizes: Species abundances in ecosystems, firm sizes in markets, city populations in countries, word counts in language, etc. A longstanding mystery of complex systems is Zipf's law, which is the empirical observation that component size decreases as the inverse of component rank -- $S \propto r^{-1}$ -- and its generalization $S \propto r^{-\alpha}$ for $\alpha \ge 0$. Herbert Simon's 1955 theoretical rich-get-richer mechanism for system growth has prevailed as capturing the essential process. But Simon's analysis is in fact flawed: In the limit of zero innovation, the model leads to a winner-takes-all system with $\alpha \rightarrow \infty$, rather than $\alpha \rightarrow 1$. Here, for pure rich-get-richer systems, we derive the time-dependent innovation rate $\rho_t$ that correctly produces power-law size rankings across all $\alpha \ge 0$. To produce Zipf's law, we uncover that $\rho_t$ must decay as the inverse of the log of the number of types, $1/\ln N$. We then show that our time-dependent innovation rate governs type emergence in any system obeying a power-law size-ranking, independent of the underlying mechanism. We demonstrate agreement between our model's output and word rankings in a collection of famous novels, while Simon's model fails. Going forward, our dynamic innovation rate mechanism provides the fundamental, Drosophila-like model for all rich-get-richer systems.

==> makepackage <==
#!/bin/sh
echo "creating $1-arxiv.tgz..." 1>&2;
cd package;

mkdir -p anc

\cp ~/work/stories/2020-08gutenberg-jane-austen/figures/figallotaxonometer9000-jane-austen-1grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf
\cp ~/work/stories/2020-08gutenberg-jane-austen/figures/figallotaxonometer9000-jane-austen-2grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf
\cp ~/work/stories/2020-08gutenberg-jane-austen/figures/figallotaxonometer9000-jane-austen-3grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf

\cp ~/work/stories/2020-01story-wrangler-rtd/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-1grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-twitter-1-grams.pdf
\cp ~/work/stories/2020-01story-wrangler-rtd/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-2grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-twitter-2-grams.pdf
\cp ~/work/stories/2020-01story-wrangler-rtd/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-3grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-twitter-3-grams.pdf

\cp ~/work/ecology/2019-11barro-colorado-trees-35-years/figures/figallotaxonometer9000-1985-2015-barro-colorado003-ptd-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf


\cp anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf \
    flipbooks/S1-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf \
    flipbooks/S2-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf \
    flipbooks/S3-flipbook-probability-divergence.pdf

\cp anc/allotaxonometer-flipbook-4-probability-divergence-twitter-1-grams.pdf \
    flipbooks/S4-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-5-probability-divergence-twitter-2-grams.pdf \
    flipbooks/S5-flipbook-probability-divergence.pdf
    
\cp anc/allotaxonometer-flipbook-6-probability-divergence-twitter-3-grams.pdf \
    flipbooks/S6-flipbook-probability-divergence.pdf
    

\cp anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf \
    flipbooks/S7-flipbook-probability-divergence.pdf
    



tar cvfzph ../$1-arxiv.tgz fig[0-9]*.pdf *revtex4-combined.tex anc/* 1>&2;



==> makepackage-arxiv <==
#!/bin/sh
echo "creating $1-arxiv.tgz..." 1>&2;

cd package;

mkdir -p anc

# clean anything if there
\rm anc/*


# jane austen
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-1grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-2grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-3grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf

# twitter
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-1grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-4-probability-divergence-twitter-1-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-2grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-5-probability-divergence-twitter-2-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-3grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-6-probability-divergence-twitter-3-grams.pdf

# barro colorado island
\cp ../figures/2019-11barro-colorado-trees-35-years/flipbooks/figallotaxonometer9000-1985-2015-barro-colorado003-ptd-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf

## tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex anc/ 1>&2;
tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex 1>&2;

cd ..



==> makepackage-no-bibtex <==
#!/bin/sh
echo "creating $1-arxiv.tgz..." 1>&2;

cd package;

mkdir -p anc

# clean anything if there
\rm anc/*


# jane austen
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-1grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-1-probability-divergence-pride-and-prejudice-1-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-2grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-2-probability-divergence-pride-and-prejudice-2-grams.pdf
\cp ../figures/2020-08gutenberg-jane-austen/flipbooks/figallotaxonometer9000-jane-austen-3grams-ptd003-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-3-probability-divergence-pride-and-prejudice-3-grams.pdf

# twitter
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-1grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-4-probability-divergence-twitter-1-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-2grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-5-probability-divergence-twitter-2-grams.pdf
\cp ../figures/2020-01story-wrangler-rtd/figallotaxonometer9000/figallotaxonometer9000-2020-03-12-2020-05-30-story-wrangler-3grams-all-prob-div_combined_noname.pdf \
    anc/allotaxonometer-flipbook-6-probability-divergence-twitter-3-grams.pdf

# barro colorado island
\cp ../figures/2019-11barro-colorado-trees-35-years/flipbooks/figallotaxonometer9000-1985-2015-barro-colorado003-ptd-alphasweep_combined.pdf \
    anc/allotaxonometer-flipbook-7-probability-turbulence-divergence-barro-colorado-island.pdf

## tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex anc/ 1>&2;
tar cvfzph ../$1-arxiv.tgz fig[0-9][0-9]*.pdf *revtex4-combined.tex 1>&2;

cd ..



==> package-arxiv <==
#!/bin/sh
echo "creating probability-divergence-manuscript-arxiv.tgz..." 1>&2;

tar cvfzph \
    probability-divergence-manuscript-arxiv.tgz \
    probability-divergence-manuscript.tex \
    probability-divergence-manuscript.*.tex \
    probability-divergence-manuscript.bbl \
    probability-divergence.*.tex \
    probability-divergence.bib \
    figures/localized/*





==> rich-get-richer-complete-manuscript.settings.tex <==
\newcommand{\filenamebase}{rich-get-richer-complete}


==> rich-get-richer-complete.author.tex <==
\author{
\firstname{Pablo}
\surname{Rosillo Rodes}
}
\email{???}

\affiliation{
    ???
}

\author{
\firstname{Laurent}
\surname{Hebert-Dufresne}
}

\email{laurent.hebert-dufresne@uvm.edu}

\affiliation{
  Department of Computer Science,
  Vermont Complex Systems Institute,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Center,
  University of Vermont,
  Burlington,
  VT 05405,
  US
}

\affiliation{
  Santa Fe Institute,
  1399 Hyde Park Rd,
  Santa Fe,
  NM 87501,
  US
}

\author{
\firstname{Julia Witte}
\surname{Zimmerman}
}
\email{julia.zimmerman@uvm.edu}
\affiliation{
        Computational Story Lab,\\
        Vermont Complex Systems Institute,\\
        University of Vermont,\\
        Burlington, VT 05405, USA
}

\author{
\firstname{Peter Sheridan}
\surname{Dodds}
}
\email{peter.dodds@uvm.edu}

\affiliation{
  Department of Computer Science,
  Vermont Complex Systems Institute,
  MassMutual Center of Excellence for Complex Systems and Data Science,
  Vermont Advanced Computing Center,
  University of Vermont,
  Burlington,
  VT 05405,
  US
}

\affiliation{
  Computational Story Lab,
  University of Vermont,
  Burlington,
  VT 05405,
  US
}

\affiliation{
  Santa Fe Institute,
  1399 Hyde Park Rd,
  Santa Fe,
  NM 87501,
  US
}

==> rich-get-richer-complete.biblio.tex <==
\bibliography{\filenamebase}


==> rich-get-richer-complete.changelog.tex <==
%% for arXivs of the various stripes

\todo{Notes on what has changed}


==> rich-get-richer-complete.contributions.tex <==
Who did what.


==> rich-get-richer-complete.data_availability.tex <==
\section*{DATA AVAILABILITY STATEMENT}

The codes for the simulations are available online (ref to github repo).

\todo{github repo}

==> rich-get-richer-complete.methods.tex <==
\section{Methods}
\label{sec:papertag.methods}






==> rich-get-richer-complete.nutshell.tex <==
\todo{Write a 1--3 sentence nutshell (logline)}



==> rich-get-richer-complete.outtakes.tex <==
\section{Introduction}
\label{sec:rich-get-richer-complete.introduction}



\begin{textblock}
\item
Putatively universal statistical regularities play a central role in complex systems. Prominent among these ubiquities is the power law, which relates a given quantity (e.g., the size of an element, $\typesize$) with a variable (e.g., the ordered rank of an element, $\rank$)\footnote{\textit{Rank} and \textit{size} are naturally central to the behavior of the model we describe, and we use them throughout the paper. However, these variables could, as noted here, represent other concepts with a power-law relationship.} such that
\begin{equation}
    S \sim r^{-\alpha}.
\end{equation}
\item
Power laws are observed throughout nature, from Zipf's law in human and animal communication~\cite{zipf1946, altmann2016, arnon2025} and heavy-tailed ecological patterns~\cite{camacho2001} to scale-free networks~\cite{barabasi1999} and diverse social systems, including the socioeconomic~\cite{serrano2003, pinto2012, gabaix2016, gaillard2023} and the sociotechnical~\cite{merton1988matthewII,Redner1998, albert1999}. Although their empirical universality has been questioned~\cite{broido2019, gerlach2019}, power laws are inarguably widespread, motivating extensive efforts to understand their origins and implications. Nevertheless, a fundamental understanding of why they emerge consistently across diverse systems remains elusive.
\end{textblock}

\begin{textblock}
\item
Many generative mechanisms have been proposed to produce power-law relationships (see~\cite{mitzenmacher2004, newman2005, roman2022, holehouse2025} and references therein). Simon's model~\cite{simon1955a}, one of the earliest and simplest of these models, built on the earlier work of Yule~\cite{yule1925a} to provide a simple mechanistic explanation for power-law size rankings via a ``rich-get-richer'' process.
The ``rich-get-richer'' mechanism is an intuitive one, with popular metaphors and idioms attesting to its productivity in cognitive and physical realms.\footnote{Examples include several Biblical iterations, one of Martial's \textit{Epigrams}, and, depending on context, phrases such as ``success breeds success'', ``it takes money to make money'', and ``standing on the shoulders of giants''~\cite{merton1988matthewII} 
(see, in particular, Merton's excellent footnote~7). Enduring imagery also evokes rich-get-richer phenomena, such as dragon hoards, scarab beetles rolling dung, and snowballs rolling downhill.}

\item 
Simon's model realizes its rich-get-richer process in this way: 
At each step, a single new element (token) is added to the system, either as a novel type with probability $\innovationprob$, or as an additional instance of an existing type with probability $1-\innovationprob$, weighted by the current frequency of each type. The resulting size-rank distribution for the types can---under conditions to be discussed---follow a power law.
\end{textblock}

\begin{figure}[t]

  \includegraphics[width=\columnwidth]{figures/localized/figrich_get_richer_simon_model_failure100_001_T08_noname.pdf}
  
  \caption{Simulations of Simon's model fail to reproduce the size–rank distribution  $\typesize_{\rank,\rgrtime,\sizerankingexponent}$ in the zero innovation limit. As $\innovationprob \to 0$ (\textbf{A}--\textbf{C}), the distribution fails to approach a power law with $\sizerankingexponent = 1 - \innovationprob \to 1$. Instead, the first-mover advantage dominates and overestimates $\typesize_{0,\rgrtime,\sizerankingexponent}$ in a factor of $1/\innovationprob$. This effect intensifies as the innovation probability decreases, arriving at $\sizerankingexponent \rightarrow \infty$ when $\rho = 0$ (\textbf{D}).}


  \label{fig:rich-get-richer-complete.simon-failure}
  
\end{figure}

\begin{textblock}
\item
    A key feature of Simon's model is the linear growth of the size of the system. At every time step, exactly one token is added, so that the total number of elements present is equal to the elapsed time, $t$. In this sense, ``time'' does not represent the physical or continuous passage of time but rather a count of cumulative events. For example, when sampling words from a book, the number of words that have been read plays the role of $t$, i.e., after $t$ steps, the text contains exactly $t$ tokens.
\end{textblock}

\begin{textblock}
\item
    The intuitive appeal and simplicity of Simon's model make it a compelling baseline for studying the emergence of power-law distributions. However, as we show in Fig.~\ref{fig:rich-get-richer-complete.simon-failure}, this formulation also carries important limitations, especially in the $\alpha = 1$ limit. 
    
\item 
First, the mechanism is unable to reproduce power laws with $\alpha\geq 1$. The average element size in Simon's model is given by $\langle s \rangle = t / (\innovationprob t)$. Here, $\langle s \rangle$ is always finite. In the case of $\alpha \geq 1$, which corresponds to $\gamma \leq 2$ in the frequency-size representation\footnote{
We may connect a power-law size distribution $P(k)\sim k^{-\gamma}$ to the corresponding Zipf's law for its size-rank relation $S_r \sim r^{-\sizerankingexponent}$ through the complementary cumulative distribution
$P_{>}(k)=\int_{s=k}^{\infty}\mathrm{d}s\,P(s)\sim k^{-\gamma+1}$.
For a system with $N$ elements, $N\,P_{>}(k)$ estimates the number of types with size greater or equal than $k$. $N\,P_{>}(k)$ is then the rank $r$ of the type of size $S_r$, and we have
$r \simeq N\,P_{>}(S_r) \sim N\,S_r^{-\gamma+1}$.
Because $S_r \sim r^{-\sizerankingexponent}$, we have $\gamma = 1 + 1/\sizerankingexponent$ and $\sizerankingexponent = 1 - \innovationprob$.
}, $\langle s \rangle$ is not defined. Thus, Simon's model cannot be used to explore $\sizerankingexponent \geq 1$.



Second, $\sizerankingexponent \rightarrow 1$ leads to $\innovationprob \rightarrow 0$, dramatically amplifying the first-mover advantage~\cite{dodds2017pre}.
\end{textblock}

\begin{textblock}
\item 
While a first-mover advantage is inherent to Simon's model, we demonstrate that the typical formulation of Simon's model fails to produce its intended power-law behavior, exaggerating the first-mover advantage. We correct the model's behavior by introducing a dynamic innovation rate, which generalizes the model to produce any possible power-law size-rank distribution. Furthermore, we show that this innovation rate is reproduced by the mere observation of \textit{any} finite growth system obeying a power-law size-ranking, regardless of the underlying dynamics of the system.

\end{textblock}

\begin{center}
    \textbf{Storyline}
\end{center}

\begin{textblock}
\item 
    In Section~\ref{sec:rich-get-richer-complete.failure}, we formalize the error in the traditional formulation of Simon's model as an amplification of the first-mover advantage. Section~\ref{sec:rich-get-richer-complete.generalized-model} then introduces our proposal of a generalized innovation rate, which corrects the traditional formulation and extends it to include \textit{all} possible power laws. Finally, in Section~\ref{sec:rich-get-richer-complete.sampling}, we demonstrate that this generalized innovation rate arises not only from the mechanistic model that we propose here but also characterizes the rate at which the set of types expands in \textit{any} sample drawn from a power-law distribution, regardless of the underlying generative process. In other words, any system described by a power-law distribution will also adhere to our generalized innovation rate, not just those systems explicable by rich-get-richer processes.

\end{textblock}


\todo{PSD: full work through}

\todo{PRR and PSD: Finish up showing errors in Simon's analysis; material in appendix with clear explanation in main text. PRR Update: wrote Appendix A4}

\todo{Emphasize: Generalized innovation rate rather than two spliced together}

\todo{Explain first mover advantage better}

\todo{Better motivation overall}

\todo{Discuss Zanette and Montemurro, 2005 paper}

\todo{Simon: First mover takes all}
e



Draft abstract:


Universal statistical regularities, such as power-
law distributions, are central to the study of complex systems. 
Numerous generative mechanisms have been proposed to explain the emergence of power laws across disparate systems, with Simon’s model being among the earliest and most influential. 


%% However, Simon’s formulation is restricted to a range where the mean size of the elements in the system is defined. 

This is a mathematical truth but does not provide intuition. 

%% This prevents the mechanism from producing power laws of the form $\typesize_{r} \sim r^{-\alpha}$ with $\alpha \geq 1$. 

Not the issue. 

Notes: Try to avoid "In addition"

"preferential attachment" is a poor term, however widespread it is. Preferential in what way? The scale-free paper was not a good one. Even "scale-free netorks" is a poor term.

%% In addition, due to its inherent linear preferential attachment, Simon's model produces a strong first-mover advantage. To resolve these issues, we introduce a dynamic innovation rate that generalizes the model and extends it to account for the full range of power-law behaviors. 

We further show that this generalized innovation rate is not only a property of the mechanistic model but also governs the growth rate of types in any system governed by a power-law distribution, regardless of the underlying generative process. 

This framework recovers well-known empirical patterns, such as Heaps’ law, and provides new insights into the mechanisms that drive power-law phenomena in fields including ecology, linguistics, and socio-economic systems.



\item
  We determine how the number of distinct types changes
  as we move from the
  $\rgrindex$th
  to the 
  $(\rgrindex+1)$th
  size-rank distribution:
  \begin{equation}
    1
    =
    (\rgrindex+1)
    -
    \rgrindex
    \sim
    \frac{
    \Ndistincttypesfn{\rgrindex+1}{\rankdistexponent}^{\rankdistexponent}
    }{
      1 - \rankdistexponent
    }
    \left[
      \Ndistincttypesfn{\rgrindex+1}{\rankdistexponent}^{1-\rankdistexponent}
      -
      1
    \right]
    -
    \frac{
      \Ndistincttypesfn{\rgrindex}{\rankdistexponent}^{\rankdistexponent}
    }{
      1 - \rankdistexponent
    }
    \left[
      \Ndistincttypesfn{\rgrindex}{\rankdistexponent}^{1-\rankdistexponent}
      -
      1
    \right].
    \label{eq:rich-get-richer-complete.Ni-change}
  \end{equation}


\item 
  \begin{equation}
    \typeinittime
    \typesize_{\rank,\rgrtime}
    \sim    
    \frac{
      (\rankdistexponent - 1)
      \,
      \rgrtime
    }{
      \rank^{\rankdistexponent}
    },
    \label{eq:rich-get-richer-complete.size-rank-distribuion-high-alpha-full}
  \end{equation}
\end{textblock}
\begin{textblock}
\item
  Because when the $\rank$th type first appears
  at $\typeinittime$,
  it is also the
  $\Ndistincttypes$th type
  at $\typeinittime$,
  we can write
\item 
  \begin{equation}
    \typeinittime
    \propto
    \Ndistincttypesfn{\typeinittime}^{\rankdistexponent}
    \label{eq:rich-get-richer-complete.tinit-Nt}
  \end{equation}
\item
  Interpolating to general $\rgrtime$,
  and inverting,
  we retrieve Heaps' law for
  $
  \rankdistexponent
  \gg
  1
  $:
\item 
  \begin{equation}
    \Ndistincttypes
    \propto
    \rgrtime^{
      \frac{
        1
      }{
        \rankdistexponent
      }
    }.
    \label{eq:rich-get-richer-complete.N-t-highalpha}
  \end{equation}
\item
  Requiring also that
  $
  \typesize_{1,\rgrtime}
  \sim
  \Ndistincttypes^{-\rankdistexponent}
  $
  (Eq.~\ref{eq:rich-get-richer-complete.size-rank-norm-check-low-alpha}),
  we have:
\item
  ?? pears at time $\typeinittime$,
  the number of distinct types at that time is
\item 
  $
  \Ndistincttypesfn{\typeinittime}
  =
  \rank.
  $
\item
  We then obtain the innovation rate's behavior
  for
  $
  \rgrtime
  \rightarrow
  \infty
  $
  and
  $\rankdistexponent
  \gg
  1
  $:
  \end{textblock}
\begin{equation}
  \innovationrate
  =
  \frac{
    \dee \Ndistincttypes
  }{
    \dee \rgrtime
  }
  \propto
  \rgrtime^{
    -
    \left(
    1
    -
    \frac{
      1
    }{
      \rankdistexponent
    }
    \right)
  }
  =
  \Ndistincttypes^{-(\rankdistexponent-1)}.
  \label{eq:rich-get-richer-complete.innovation-rate-high-alpha}
\end{equation}

\todo{Get the right normalization and then construction rho t}



  which correctly gives us Heaps' law for
  $\rankdistexponent \ll 1$:
\item 
  \begin{equation}
    \Ndistincttypes
    \sim
    (1 - \rankdistexponent)
    \rgrtime
    =
    \innovationprob
    \rgrtime
    \label{eq:rich-get-richer-complete.heaps-law-low-alpha}
  \end{equation}


\item
  Substituting for $\rank$ in Eq.~\ref{eq:rich-get-richer-complete.growing-initiation-time},
  interpolating to general $\rgrtime$,
  and inverting,
  we retrieve Heaps' law for
  $
  \rankdistexponent
  \gg
  1
  $:
\item 
\begin{equation}
  \Ndistincttypes
  \propto
  \rgrtime^{
    \frac{
      1
    }{
      \rankdistexponent
    }
  }.
  \label{eq:rich-get-richer-complete.N-t-highalpha}
\end{equation}


\item 
\begin{equation}
  \typeinittime
  \sim
  \frac{
    \rgrtime
  }{
    \Ndistincttypesfn{\typeinittime}
  }
  \rank^{\rankdistexponent}
  \
  \textnormal{for}
  \
  \rankdistexponent
  \gg
  1.
  \label{eq:rich-get-richer-complete.growing-initiation-time}
\end{equation}


\begin{textblock}
\item
  We write the number of distinct types at time
  $\rgrtime$
  as
  $\Ndistincttypes$.
\item
  
\item
\end{textblock}
\begin{equation}
  \Ndistincttypes
  \propto
  \rgrtime^{\Ntypesexponent}
  =
  \left\{
  \begin{array}{l}
    \rgrtime^{1}
    \,
    \textnormal{for}
    \,
    \rankdistexponent \le 1,
    \\
    \rgrtime^{1/\rankdistexponent}
    \,
    \textnormal{for}
    \,
    \rankdistexponent > 1.
  \end{array}
  \right.
  \label{eq:rich-get-richer-complete.heaps-law}
\end{equation}

